Interfering-or-not-interfering quantum key distribution with advantage distillation

Interfering-or-not-interfering quantum key distribution (INI-QKD) is an innovative protocol whose performance surpasses existing twin-field protocol variants. In this study, we introduce an additional step of advantage distillation (AD) after the quantum communication phase to further enhance its performance. Through the AD the raw key is partitioned into small blocks of bits to identify highly correlated bit pairs. We numerically compute the optimal partitioning for different realistic conditions. Our results show that by employing the advantage distillation the transmission distance is significantly increased and thus can potentially improve the secret key rate of INI-QKD. This in particular is most prominent in the presence of high polarization misalignment error rates and considerable phase mismatch, all without altering the experimental setup of the protocol.

==> tfqkd.tex <==
@article{bennett2014quantum,
  title={Quantum cryptography: Public key distribution and coin tossing},
  author={Bennett, Charles H and Brassard, Gilles},
  journal={Theor. Comput. Sci.},
  volume={560},
  pages={7--11},
  year={2014},
  doi = {https://doi.org/10.1016/j.tcs.2014.05.025},
  url = {https://www.sciencedirect.com/science/article/pii/S0304397514004241},
  publisher={Elsevier}
}

@article{bennett1992experimental,
  title={Experimental quantum cryptography},
  author={Bennett, Charles H and Bessette, Fran{\c{c}}ois and Brassard, Gilles and Salvail, Louis and Smolin, John},
  journal={J. Cryptol.},
  volume={5},
  pages={3--28},
  year={1992},
  doi = {https://doi.org/10.1007/BF00191318}, 
  url = {https://link.springer.com/article/10.1007/BF00191318#citeas},
  publisher={Springer}
}
@article{ekert1991quantum,
  title={Quantum cryptography based on Bell’s theorem},
  author={Ekert, Artur K},
  journal={Phys. Rev. Lett.},
  volume={67},
  number={6},
  pages={661},
  year={1991},
  doi = {10.1103/PhysRevLett.67.661},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.67.661},
  publisher={APS}
}
@article{lo1999unconditional,
  title={Unconditional security of quantum key distribution over arbitrarily long distances},
  author={Lo, Hoi-Kwong and Chau, Hoi Fung},
  journal={Science},
  volume={283},
  number={5410},
  pages={2050--2056},
  year={1999},
  doi = {DOI: 10.1126/science.283.5410.2050},
  url = {https://www.science.org/doi/10.1126/science.283.5410.2050},
  publisher={American Association for the Advancement of Science}
}
@article{shor2000simple,
  title={Simple proof of security of the BB84 quantum key distribution protocol},
  author={Shor, Peter W and Preskill, John},
  journal={Phys. Rev. Lett.},
  volume={85},
  number={2},
  pages={441},
  year={2000},
  doi = {https://doi.org/10.1103/PhysRevLett.85.441},
  url = {https://journals.aps.org/prl/abstract/10.1103/PhysRevLett.85.441},
  publisher={APS}
}
@article{mayers2001unconditional,
  title={Unconditional security in quantum cryptography},
  author={Mayers, Dominic},
  journal={JACM},
  volume={48},
  number={3},
  pages={351--406},
  year={2001},
  doi = {https://doi.org/10.1145/382780.38278},
  url = {https://dl.acm.org/doi/abs/10.1145/382780.382781},
  publisher={ACM New York, NY, USA}
}
@article{diamanti2016practical,
  title={Practical challenges in quantum key distribution},
  author={Diamanti, Eleni and Lo, Hoi-Kwong and Qi, Bing and Yuan, Zhiliang},
  journal={npj Quantum Inf.},
  volume={2},
  number={1},
  pages={1--12},
  year={2016},
  doi = {https://doi.org/10.1038/npjqi.2016.25},
  url = {https://www.nature.com/articles/npjqi201625},
  publisher={Nature Publishing Group}
}
@article{liu2023experimental,
  title={Experimental twin-field quantum key distribution over 1000 km fiber distance},
  author={Liu, Yang and Zhang, Wei-Jun and Jiang, Cong and others},
  journal={Phys. Rev. Lett.},
  volume={130},
  number={21},
  pages={210801},
  year={2023},
  doi = {10.1103/PhysRevLett.130.210801},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.130.210801},
  publisher={APS}
}
@article{sun2022review,
  title={A review of security evaluation of practical quantum key distribution system},
  author={Sun, Shihai and Huang, Anqi},
  journal={Entropy},
  volume={24},
  number={2},
  pages={260},
  year={2022},
  doi = {https://doi.org/10.1038/npjqi.2016.25},
  url = {https://www.mdpi.com/1099-4300/24/2/260},
  publisher={MDPI}
}
@article{He2022,
  title = {Teleportation of discrete-variable qubits via continuous-variable lossy channels},
  author = {He, Mingjian and Malaney, Robert and Aguinaldo, Ryan},
  journal = {Phys. Rev. A},
  volume = {105},
  issue = {6},
  pages = {062407},
  numpages = {11},
  year = {2022},
  month = {Jun},
  doi = {10.1103/PhysRevA.105.062407},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.105.062407},
  publisher = {American Physical Society},
}
@inproceedings{mayers1998quantum,
  title={Quantum cryptography with imperfect apparatus},
  author={Mayers, Dominic and Yao, Andrew},
  booktitle={Proc. 39th Annu. Symp. Found. Comput. Sci. (Cat. No. 98CB36280)},
  pages={503--509},
  year={1998},
  doi={10.1109/SFCS.1998.743501},
  url = {https://ieeexplore.ieee.org/document/743501},
  organization={IEEE}
}
@article{barrett2005no,
  title={No signaling and quantum key distribution},
  author={Barrett, Jonathan and Hardy, Lucien and Kent, Adrian},
  journal={Phys. Rev. Lett.},
  volume={95},
  number={1},
  pages={010503},
  year={2005},
  doi = {https://doi.org/10.1103/PhysRevLett.95.010503},
  url = {https://journals.aps.org/prl/abstract/10.1103/PhysRevLett.95.010503},
  publisher={APS}
}
@article{pirandola2020advances,
  title={Advances in quantum cryptography},
  author={Pirandola, Stefano and Andersen, Ulrik L and others},
  journal={Adv. Opt. Photonics},
  volume={12},
  number={4},
  pages={1012--1236},
  year={2020},
  doi = {https://doi.org/10.1364/AOP.361502},
  url = {https://opg.optica.org/aop/abstract.cfm?URI=aop-12-4-1012},
  publisher={Optica Publishing Group}
}
@article{xu2020secure,
  title={Secure quantum key distribution with realistic devices},
  author={Xu, Feihu and Ma, Xiongfeng and Zhang, Qiang and Lo, Hoi-Kwong and Pan, Jian-Wei},
  journal={Rev. Mod. Phys.},
  volume={92},
  number={2},
  pages={025002},
  year={2020},
  doi ={https://doi.org/10.1364/AOP.361502},
  url = {https://opg.optica.org/viewmedia.cfm?r=1&rwjcode=aop&uri=aop-12-4-1012},
  publisher={APS}
}
@article{Rozpedek2018,
  title = {Optimizing practical entanglement distillation},
  author = {Rozp\ifmmode \mbox{\k{e}}\else \k{e}\fi{}dek, Filip and Schiet, Thomas and Thinh, Le Phuc and Elkouss, David and Doherty, Andrew C. and Wehner, Stephanie},
  journal = {Phys. Rev. A},
  volume = {97},
  issue = {6},
  pages = {062333},
  numpages = {32},
  year = {2018},
  month = {Jun},
  doi = {10.1103/PhysRevA.97.062333},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.97.062333},
  publisher = {APS}
}
@article{Ma2018,
  title = {Phase-matching quantum key distribution},
  author = {Ma, X. and Zeng, P. and Zhou, H.},
  journal = {Phys. Rev. X},
  volume = {8},
  number = {3},
  pages = {031043},
  year = {2018},
  doi = {https://doi.org/10.1103/PhysRevX.8.031043},
  url = {https://journals.aps.org/prx/abstract/10.1103/PhysRevX.8.031043},
  publisher = {APS}
}

@article{Tamaki2018,
  title = {Information theoretic security of quantum key distribution overcoming the repeaterless secret key capacity bound},
  author = {Tamaki, K. and Lo, H.-K. and Wang, W. and Lucamarini, M.},
  journal = {arXiv},
  year = {2018},
  eprint = {1805.05511},
  url = {https://arxiv.org/abs/1805.05511},
  publisher = {arXiv}
}

@article{Wang2018,
  title = {Twin-field quantum key distribution with large misalignment error},
  author = {Wang, X.-B. and Yu, Z.-W. and Hu, X.-L.},
  journal = {Phys. Rev. A},
  volume = {98},
  number = {6},
  pages = {062323},
  year = {2018},
  doi = {https://doi.org/10.1103/PhysRevA.98.062323},
  url = {https://journals.aps.org/pra/abstract/10.1103/PhysRevA.98.062323},
  publisher = {APS}
}

@article{Cui2019,
  title = {Twin-field quantum key distribution without phase postselection},
  author = {Cui, C. and Yin, Z.-Q. and Wang, R. and Chen, W. and Wang, S. and Guo, G.-C. and Han, Z.-F.},
  journal = {Phys. Rev. Appl.},
  volume = {11},
  number = {3},
  pages = {034053},
  year = {2019},
  doi = {https://doi.org/10.1103/PhysRevApplied.11.034053},
  url = {https://journals.aps.org/prapplied/abstract/10.1103/PhysRevApplied.11.034053},
  publisher = {APS}
}

@article{Curty2019,
  title = {Simple security proof of twin-field type quantum key distribution protocol},
  author = {Curty, M. and Azuma, K. and Lo, H.-K.},
  journal = {npj Quantum Inf.},
  volume = {5},
  pages = {64},
  year = {2019},
  doi = {https://doi.org/10.1038/s41534-019-0175-6},
  url = {https://www.nature.com/articles/s41534-019-0175-6},
  publisher = {Springer Nature}
}

@article{Lin2018,
  title = {Simple security analysis of phase-matching measurement-device-independent quantum key distribution},
  author = {Lin, J. and Lütkenhaus, N.},
  journal = {Phys. Rev. A},
  volume = {98},
  number = {4},
  pages = {042332},
  year = {2018},
  doi = {https://doi.org/10.1103/PhysRevA.98.042332},
  url = {https://journals.aps.org/pra/abstract/10.1103/PhysRevA.98.042332},
  publisher = {APS}
}

@article{Yin2019,
  title = {Measurement-device-independent twin-field quantum key distribution},
  author = {Yin, H.-L. and Fu, Y.},
  journal = {Sci. Rep.},
  volume = {9},
  pages = {3045},
  year = {2019},
  doi = {https://doi.org/10.1038/s41598-019-39350-1},
  url = {https://www.nature.com/articles/s41598-019-39350-1},
  publisher = {Springer Nature}
}

@article{Wang2020,
  title = {Optimized protocol for twin-field quantum key distribution},
  author = {Wang, R. and Yin, Z.-Q. and Lu, F.-Y. and Wang, S. and Chen, W. and Zhang, C.-M. and Guo, G.-C. and Han, Z.-F.},
  journal = {Commun. Phys.},
  volume = {3},
  pages = {149},
  year = {2020},
  doi = {https://doi.org/10.1038/s42005-020-00418-7},
  url = {https://www.nature.com/articles/s42005-020-00418-7},
  publisher = {Springer Nature}
}

@article{Zeng2020,
  title = {Symmetry-protected privacy: Beating the rate-distance linear bound over a noisy channel},
  author = {Zeng, P. and Wu, W. and Ma, X.},
  journal = {Phys. Rev. Appl.},
  volume = {13},
  number = {6},
  pages = {064013},
  year = {2020},
  doi = {https://doi.org/10.1103/PhysRevApplied.13.064013},
  url = {https://journals.aps.org/prapplied/abstract/10.1103/PhysRevApplied.13.064013},
  publisher = {APS}
}

@article{Xu2020,
  title = {Sending-or-not-sending twin-field quantum key distribution: Breaking the direct transmission key rate},
  author = {Xu, H. and Yu, Z.-W. and Jiang, C. and Hu, X.-L. and Wang, X.-B.},
  journal = {Phys. Rev. A},
  volume = {101},
  number = {4},
  pages = {042330},
  year = {2020},
  doi = {https://doi.org/10.1103/PhysRevA.101.042330},
  url = {https://journals.aps.org/pra/abstract/10.1103/PhysRevA.101.042330},
  publisher = {APS}
}

@article{Curras2021,
  title = {Twin-field quantum key distribution with fully discrete phase randomization},
  author = {Currás-Lorenzo, G. and Wooltorton, L. and Razavi, M.},
  journal = {Phys. Rev. Appl.},
  volume = {15},
  number = {1},
  pages = {014016},
  year = {2021},
  doi = {https://doi.org/10.1103/PhysRevApplied.15.014016},
  url = {https://journals.aps.org/prapplied/abstract/10.1103/PhysRevApplied.15.014016},
  publisher = {APS}
}

@article{Zhang2020,
  title = {Twin-field quantum key distribution with discrete-phase-randomized sources},
  author = {Zhang, C.-M. and Xu, Y.-W. and Wang, R. and Wang, Q.},
  journal = {Phys. Rev. Appl.},
  volume = {14},
  number = {6},
  pages = {064070},
  year = {2020},
  doi = {https://doi.org/10.1103/PhysRevApplied.14.064070},
  url = {https://journals.aps.org/prapplied/abstract/10.1103/PhysRevApplied.14.064070},
  publisher = {APS}
}

@article{Jiang2020,
  title = {Sending-or-not-sending twin-field quantum key distribution with discrete-phase-randomized weak coherent states},
  author = {Jiang, C. and Yu, Z.-W. and Hu, X.-L. and Wang, X.-B.},
  journal = {Phys. Rev. Res.},
  volume = {2},
  number = {4},
  pages = {043304},
  year = {2020},
  doi = {https://doi.org/10.1103/PhysRevResearch.2.043304},
  url = {https://journals.aps.org/prresearch/abstract/10.1103/PhysRevResearch.2.043304},
  publisher = {APS}
}

@article{Zhang2021,
  title = {Phase-matching quantum key distribution with discrete phase randomization},
  author = {Zhang, X. and Wang, Y. and Jiang, M. and Lu, Y. and Li, H. and Zhou, C. and Bao, W.},
  journal = {Entropy},
  volume = {23},
  number = {4},
  pages = {508},
  year = {2021},
  doi = {https://doi.org/10.3390/e23040508},
  url = {https://www.mdpi.com/1099-4300/23/4/508},
  publisher = {MDPI}
}


@article{Xu2021,
  title = {Discrete-phase-randomized twin-field quantum key distribution without phase postselection in the test mode},
  author = {Xu, Y.-W. and Wang, R. and Zhang, C.-M.},
  journal = {Quantum Inf. Process.},
  volume = {20},
  number = {6},
  pages = {199},
  year = {2021},
  doi = {https://doi.org/10.1007/s11128-021-03147-1},
  url = {https://link.springer.com/article/10.1007/s11128-021-03147-1},
  publisher = {Springer}
}

@article{Hu2022,
  title = {Universal approach to sending-or-not-sending twin field quantum key distribution},
  author = {Hu, X.-L. and Jiang, C. and Yu, Z.-W. and Wang, X.-B.},
  journal = {Quantum Sci. Technol.},
  volume = {7},
  number = {4},
  pages = {045031},
  year = {2022},
  doi = {https://doi.org/10.1088/2058-9565/ac7c36},
  url = {https://iopscience.iop.org/article/10.1088/2058-9565/ac7c36},
  publisher = {IOP Publishing}
}

@article{vagniluca2020efficient,
  title={Efficient time-bin encoding for practical high-dimensional quantum key distribution},
  author={Vagniluca, Ilaria and Da Lio, Beatrice and Rusca, Davide and others},
  journal={Phys. Rev. Appl.},
  volume={14},
  number={1},
  pages={014051},
  year={2020},
  doi = {https://doi.org/10.1103/PhysRevApplied.14.014051},
  url = {https://journals.aps.org/prapplied/abstract/10.1103/PhysRevApplied.14.014051},
  publisher={APS}
}
@article{Kumar2023,
  title = {Success probability and performance optimization in non-Gaussian continuous-variable quantum teleportation},
  author = {Kumar, Chandan and Arora, Shikhar},
  journal = {Phys. Rev. A},
  volume = {107},
  issue = {1},
  pages = {012418},
  numpages = {15},
  year = {2023},
  month = {Jan},
  doi = {10.1103/PhysRevA.107.012418},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.107.012418},
  publisher = {APS}
}
@article{lo2012measurement,
  title={Measurement-device-independent quantum key distribution},
  author={Lo, Hoi-Kwong and Curty, Marcos and Qi, Bing},
  journal={Phys. Rev. Lett.},
  volume={108},
  number={13},
  pages={130503},
  year={2012},
  doi = {10.1103/PhysRevLett.108.130503},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.108.130503},
  publisher={APS}
}
@article{braunstein2012side,
  title={Side-channel-free quantum key distribution},
  author={Braunstein, Samuel L and Pirandola, Stefano},
  journal={Phys. Rev. Lett.},
  volume={108},
  number={13},
  pages={130502},
  year={2012},
  doi = {10.1103/PhysRevLett.108.130502},
  url ={https://link.aps.org/doi/10.1103/PhysRevLett.108.130502},
  publisher={APS}
}
@article{pirandola2017fundamental,
  title={Fundamental limits of repeaterless quantum communications},
  author={Pirandola, Stefano and Laurenza, Riccardo and Ottaviani, Carlo and Banchi, Leonardo},
  journal={Nat. Commun.},
  volume={8},
  number={1},
  pages={1--15},
  year={2017},
  doi= {10.1038/ncomms15043},
  url={https://www.nature.com/articles/ncomms15043},
  publisher={Nature Publishing Group}
}
@article{lucamarini2018overcoming,
  title={Overcoming the rate--distance limit of quantum key distribution without quantum repeaters},
  author={Lucamarini, Marco and Yuan, Zhiliang L and Dynes, James F and Shields, Andrew J},
  journal={Nature},
  volume={557},
  number={7705},
  pages={400--403},
  year={2018},
  doi= {10.1038/s41586-018-0066-6},
  publisher={Nature Publishing Group UK London}
}
@article{abruzzo2013quantum,
  title={Quantum repeaters and quantum key distribution: Analysis of secret-key rates},
  author={Abruzzo, Silvestre and Bratzik, Sylvia and Bernardes, Nadja K and Kampermann, Hermann and Van Loock, Peter and Bru{\ss}, Dagmar},
  journal={Phys. Rev. A},
  volume={87},
  number={5},
  pages={052315},
  year={2013},
  doi={https://doi.org/10.1103/PhysRevA.87.052315},
  publisher={APS}
}
@article{amirloo2010quantum,
  title={Quantum key distribution over probabilistic quantum repeaters},
  author={Amirloo, Jeyran and Razavi, Mohsen and Majedi, A Hamed},
  journal={Phys. Rev. A},
  volume={82},
  number={3},
  pages={032304},
  year={2010},
  doi={https://doi.org/10.1103/PhysRevA.82.032304},
  publisher={APS}
}
@article{mardani2020continuous,
  title={Continuous-variable entanglement distillation by cascaded photon replacement},
  author={Mardani, Yasamin and Shafiei, Ali and Ghadimi, Milad and Abdi, Mehdi},
  journal={Phys. Rev. A},
  volume={102},
  number={1},
  pages={012407},
  year={2020},
  doi={https://doi.org/10.1103/PhysRevA.102.012407},
  publisher={APS}
}
@article{takeoka2014fundamental,
  title={Fundamental rate-loss tradeoff for optical quantum key distribution},
  author={Takeoka, Masahiro and Guha, Saikat and Wilde, Mark M},
  journal={Nat. Commun.},
  volume={5},
  number={1},
  pages={5235},
  year={2014},
  doi={10.1038/ncomms6235},
  publisher={Nature Publishing Group UK London}
}
@article{ma2018phase,
  title={Phase-matching quantum key distribution},
  author={Ma, Xiongfeng and Zeng, Pei and Zhou, Hongyi},
  journal={Phys. Rev. X},
  volume={8},
  number={3},
  pages={031043},
  year={2018},
  doi = {10.1103/PhysRevX.8.031043},
  publisher={APS}
}
@article{cui2019twin,
  title={Twin-field quantum key distribution without phase postselection},
  author={Cui, Chaohan and Yin, Zhen-Qiang and Wang, Rong and Chen, Wei and Wang, Shuang and Guo, Guang-Can and Han, Zheng-Fu},
  journal={Phys. Rev. Appl.},
  volume={11},
  number={3},
  pages={034053},
  year={2019},
  doi = {10.1103/PhysRevApplied.11.034053},
  publisher={APS}
}
@article{lu2019practical,
  title={Practical issues of twin-field quantum key distribution},
  author={Lu, Feng-Yu and Yin, Zhen-Qiang and Wang, Rong and others},
  journal={New J. Phys.},
  volume={21},
  number={12},
  pages={123030},
  year={2019},
  doi = {10.1088/1367-2630/ab5a97},
  publisher={IOP Publishing}
}
@article{wang2018twin,
  title={Twin-field quantum key distribution with large misalignment error},
  author={Wang, Xiang-Bin and Yu, Zong-Wen and Hu, Xiao-Long},
  journal={Phys. Rev. A},
  volume={98},
  number={6},
  pages={062323},
  year={2018},
  doi = {10.1103/PhysRevA.98.062323},
  publisher={APS}
}
@article{xu2020sending,
  title={Sending-or-not-sending twin-field quantum key distribution: Breaking the direct transmission key rate},
  author={Xu, Hai and Yu, Zong-Wen and Jiang, Cong and Hu, Xiao-Long and Wang, Xiang-Bin},
  journal={Phys. Rev. A},
  volume={101},
  number={4},
  pages={042330},
  year={2020},
  doi = {10.1103/PhysRevA.101.042330},
  publisher={APS}
}
@article{wang2019beating,
  title={Beating the fundamental rate-distance limit in a proof-of-principle quantum key distribution system},
  author={Wang, Shuang and He, De-Yong and Yin, Zhen-Qiang and others},
  journal={Phys. Rev. X},
  volume={9},
  number={2},
  pages={021046},
  year={2019},
  doi = {10.1103/PhysRevX.9.021046},
  publisher={APS}
}
@article{fang2020implementation,
  title={Implementation of quantum key distribution surpassing the linear rate-transmittance bound},
  author={Fang, Xiao-Tian and Zeng, Pei and Liu, Hui and others},
  journal={Nat. Photonics},
  volume={14},
  number={7},
  pages={422--425},
  year={2020},
  doi={10.1038/s41566-020-0599-8},
  publisher={Nature Publishing Group UK London}
}
@article{chen2020sending,
  title={Sending-or-not-sending with independent lasers: Secure twin-field quantum key distribution over 509 km},
  author={Chen, Jiu-Peng and Zhang, Chi and Liu, Yang and others},
  journal={Phys. Rev. Lett.},
  volume={124},
  number={7},
  pages={070501},
  year={2020},
  doi = {10.1103/PhysRevLett.124.070501},
  publisher={APS}
}
@article{cerf2002security,
  title={Security of quantum key distribution using d-level systems},
  author={Cerf, Nicolas J and Bourennane, Mohamed and Karlsson, Anders and Gisin, Nicolas},
  journal={Phys. Rev. Lett.},
  volume={88},
  number={12},
  pages={127902},
  year={2002},
  doi = {10.1103/PhysRevLett.88.127902},
  publisher={APS}
}
@article{bouchard2017high,
  title={High-dimensional quantum cloning and applications to quantum hacking},
  author={Bouchard, Fr{\'e}d{\'e}ric and Fickler, Robert and Boyd, Robert W and Karimi, Ebrahim},
  journal={Sci. Adv.},
  volume={3},
  number={2},
  pages={e1601915},
  year={2017},
  doi={10.1126/sciadv.1601915},
  publisher={American Association for the Advancement of Science}
}
@article{yu2024interfering,
  title={Interfering-or-not-interfering quantum key distribution},
  author={Yu, Yang and Li, Wei and Wang, Le and Zhao, Shengmei},
  journal={Phys. Rev. A},
  volume={109},
  number={5},
  pages={052609},
  year={2024},
  doi = {10.1103/PhysRevA.109.052609},
  publisher={APS}
}
@inproceedings{brassard1993secret,
  title={Secret-key reconciliation by public discussion},
  author={Brassard, Gilles and Salvail, Louis},
  booktitle={Workshop on the Theory and Application of Cryptographic Techniques},
  pages={410--423},
  year={1993},
  doi = {https://doi.org/10.1007/3-540-48285-7_35},
  url = {https://link.springer.com/chapter/10.1007/3-540-48285-7_35#citeas},
  organization={Springer}
}
@article{bennett1988privacy,
  title={Privacy amplification by public discussion},
  author={Bennett, Charles H and Brassard, Gilles and Robert, Jean-Marc},
  journal={SIAM J. Comput.},
  volume={17},
  number={2},
  pages={210--229},
  year={1988},
  doi = {https://doi.org/10.1137/0217014},
  url = {https://epubs.siam.org/doi/10.1137/0217014},
  publisher={SIAM}
}
@article{renner2008security,
  title={Security of quantum key distribution},
  author={Renner, Renato},
  journal={Int. J. Quantum Inf.},
  volume={6},
  number={01},
  pages={1--127},
  year={2008},
  doi={10.1142/S0219749908003256},
  publisher={World Scientific}
}
@article{kraus2007security,
  title={Security of quantum-key-distribution protocols using two-way classical communication or weak coherent pulses},
  author={Kraus, Barbara and Branciard, Cyril and Renner, Renato},
  journal={Phys. Rev. A},
  volume={75},
  number={1},
  pages={012316},
  year={2007},
  doi = {10.1103/PhysRevA.75.012316},
  publisher={APS}
}
@article{bae2007key,
  title={Key distillation from quantum channels using two-way communication protocols},
  author={Bae, Joonwoo and Ac{\'\i}n, Antonio},
  journal={Phys. Rev. A},
  volume={75},
  number={1},
  pages={012334},
  year={2007},
  doi = {10.1103/PhysRevA.75.012334},
  publisher={APS}
}
@article{murta2020key,
  title={Key rates for quantum key distribution protocols with asymmetric noise},
  author={Murta, Gl{\'a}ucia and Rozp{\k{e}}dek, Filip and Ribeiro, J{\'e}r{\'e}my and Elkouss, David and Wehner, Stephanie},
  journal={Phys. Rev. A},
  volume={101},
  number={6},
  pages={062321},
  year={2020},
  doi = {10.1103/PhysRevA.101.062321},
  publisher={APS}
}
@article{tan2020advantage,
  title={Advantage distillation for device-independent quantum key distribution},
  author={Tan, Ernest Y-Z and Lim, Charles C-W and Renner, Renato},
  journal={Phys. Rev. Lett.},
  volume={124},
  number={2},
  pages={020502},
  year={2020},
  doi = {10.1103/PhysRevLett.124.020502},
  publisher={APS}
}
@article{li2022improving,
  title={Improving the performance of practical decoy-state quantum key distribution with advantage distillation technology},
  author={Li, Hong-Wei and Zhang, Chun-Mei and Jiang, Mu-Sheng and Cai, Qing-Yu},
  journal={Commun. Phys.},
  volume={5},
  number={1},
  pages={53},
  year={2022},
  doi={10.1038/s42005-022-00831-4},
  publisher={Nature Publishing Group}
}
@article{wang2022phase,
  title={Phase-matching quantum key distribution with advantage distillation},
  author={Wang, Rui-Qiang and Zhang, Chun-Mei and Yin, Zhen-Qiang and others},
  journal={New J. Phys.},
  volume={24},
  number={7},
  pages={073049},
  year={2022},
  doi={10.1088/1367-2630/ac8115},
  publisher={IOP Publishing}
}
@article{jiang2023improving,
  title={Improving the performance of reference-frame-independent quantum key distribution with advantage distillation technology},
  author={Jiang, Xiao-Lei and Wang, Yang and Li, Jia-Ji and others},
  journal={Opt. Express},
  volume={31},
  number={6},
  pages={9196--9210},
  year={2023},
  doi={10.1364/OE.480570},
  publisher={Optica Publishing Group}
}
@article{zhou2024sending,
  title={Sending-or-not-sending twin-field quantum key distribution with advantage distillation},
  author={Zhou, Yao and Wang, Rui-Qiang and others},
  journal={Phys. Rev. Appl.},
  volume={21},
  number={1},
  pages={014036},
  year={2024},
  doi = {10.1103/PhysRevApplied.21.014036},
  publisher={APS}
}
@article{zhang2024discrete,
  title={Discrete-phase-randomized twin-field quantum key distribution with advantage distillation},
  author={Zhang, Chun-Mei and Wang, Zhe and Wu, Yu-Da and others},
  journal={Phys. Rev. A},
  volume={109},
  number={5},
  pages={052432},
  year={2024},
  doi = {10.1103/PhysRevA.109.052432},
  publisher={APS}
}
@article{liu2023mode,
  title={Mode-pairing quantum key distribution with advantage distillation},
  author={Liu, Xin and Luo, Di and Zhang, Zhenrong and others},
  journal={Phys. Rev. A},
  volume={107},
  number={6},
  pages={062613},
  year={2023},
  doi = {10.1103/PhysRevA.107.062613},
  publisher={APS}
}
@article{xu2013practical,
  title={Practical aspects of measurement-device-independent quantum key distribution},
  author={Xu, Feihu and Curty, Marcos and others},
  journal={New J. Phys.},
  volume={15},
  number={11},
  pages={113007},
  year={2013},
  doi = {10.1088/1367-2630/15/11/113007},
  publisher={IOP Publishing}
}
@article{zhu2023reference,
  title={Reference-frame-independent quantum key distribution with advantage distillation},
  author={Zhu, Jian-Rong and Zhang, Chun-Mei and Wang, Rong and others},
  journal={Opt. Lett.},
  volume={48},
  number={3},
  pages={542--545},
  year={2023},
  doi={/10.1364/OL.480427},
  publisher={Optica Publishing Group}
}
@article{hu2023practical,
  title={Practical measurement-device-independent quantum key distribution with advantage distillation},
  author={Hu, Li-Wen and Zhang, Chun-Mei and Li, Hong-Wei},
  journal={Quantum Inf. Process.},
  volume={22},
  number={1},
  pages={77},
  year={2023},
  doi={10.1007/s11128-022-03810-4},
  publisher={Springer}
}
@article{wang2024improving,
  title={Improving the performance of practical phase-matching quantum key distribution with advantage distillation},
  author={Wang, Zhe and Zhang, Chun-Mei and Li, Hong-Wei},
  journal={Quantum Inf. Process.},
  volume={23},
  number={4},
  pages={128},
  year={2024},
  doi={10.1007/s11128-024-04337-6},
  publisher={Springer}
}
@article{luo2024practical,
  title={Practical asynchronous measurement-device-independent quantum key distribution with advantage distillation},
  author={Luo, Di and Liu, Xin and Qin, Kaibiao and Zhang, Zhenrong and Wei, Kejin},
  journal={Phys. Rev. A},
  volume={110},
  number={2},
  pages={022605},
  year={2024},
  doi = {10.1103/PhysRevA.110.022605},
  publisher={APS}
}
@article{Maurer,
  author={Maurer, U.M.},
  journal={IEEE Trans. Inf. Theory}, 
  title={Secret key agreement by public discussion from common information}, 
  year={1993},
  volume={39},
  number={3},
  pages={733-742},
  doi={10.1109/18.256484}
}
@article{Gottesman,
  author={Gottesman, D. and Hoi-Kwong Lo},
  journal={IEEE Trans. Inf. Theory}, 
  title={Proof of security of quantum key distribution with two-way classical communications}, 
  year={2003},
  volume={49},
  number={2},
  pages={457-475},
  doi={10.1109/TIT.2002.807289}
}
@article{Ma,
  title = {Decoy-state quantum key distribution with two-way classical postprocessing},
  author = {Ma, Xiongfeng and Fung, Chi-Hang Fred and Dupuis, Fr\'ed\'eric and Chen, Kai and Tamaki, Kiyoshi and Lo, Hoi-Kwong},
  journal = {Phys. Rev. A},
  volume = {74},
  issue = {3},
  pages = {032330},
  numpages = {16},
  year = {2006},
  month = {Sep},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.74.032330},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.74.032330}
}
@article{Li2023improving,
  doi = {10.22331/q-2023-12-06-1201},
  url = {https://doi.org/10.22331/q-2023-12-06-1201},
  title = {Improving the performance of twin-field quantum key distribution with advantage distillation technology},
  author = {Li, Hong-Wei and Wang, Rui-Qiang and Zhang, Chun-Mei and Cai, Qing-Yu},
  journal = {{Quantum}},
  ISSN = {2521-327X},
  publisher = {{Verein zur F{\"{o}}rderung des Open Access Publizierens in den Quantenwissenschaften}},
  volume = {7},
  pages = {1201},
  month = Dec,
  year = {2023}
}
@article{Kraus,
  title = {Lower and Upper Bounds on the Secret-Key Rate for Quantum Key Distribution Protocols Using One-Way Classical Communication},
  author = {Kraus, B. and Gisin, N. and Renner, R.},
  journal = {Phys. Rev. Lett.},
  volume = {95},
  issue = {8},
  pages = {080501},
  numpages = {4},
  year = {2005},
  month = {Aug},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.95.080501},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.95.080501}
}



@inproceedings{mayers1998quantum,
  title={Quantum cryptography with imperfect apparatus},
  author={Mayers, Dominic and Yao, Andrew},
  booktitle={Proceedings 39th Annual Symposium on Foundations of Computer Science (Cat. No. 98CB36280)},
  pages={503--509},
  year={1998},
  doi={10.1109/SFCS.1998.743501},
  url = {https://ieeexplore.ieee.org/document/743501},
  organization={IEEE}
}
@article{barrett2005no,
  title={No signaling and quantum key distribution},
  author={Barrett, Jonathan and Hardy, Lucien and Kent, Adrian},
  journal={Physical review letters},
  volume={95},
  number={1},
  pages={010503},
  year={2005},
  doi = {https://doi.org/10.1103/PhysRevLett.95.010503},
  url = {https://journals.aps.org/prl/abstract/10.1103/PhysRevLett.95.010503},
  publisher={APS}
}

@article{vagniluca2020efficient,
  title={Efficient time-bin encoding for practical high-dimensional quantum key distribution},
  author={Vagniluca, Ilaria and Da Lio, Beatrice and Rusca, Davide and Cozzolino, Daniele and Ding, Yunhong and Zbinden, Hugo and Zavatta, Alessandro and Oxenl{\o}we, Leif K and Bacco, Davide},
  journal={Physical Review Applied},
  volume={14},
  number={1},
  pages={014051},
  year={2020},
  doi = {https://doi.org/10.1103/PhysRevApplied.14.014051},
  url = {https://journals.aps.org/prapplied/abstract/10.1103/PhysRevApplied.14.014051},
  publisher={APS}
}

@article{ma2018phase,
  title={Phase-matching quantum key distribution},
  author={Ma, Xiongfeng and Zeng, Pei and Zhou, Hongyi},
  journal={Physical Review X},
  volume={8},
  number={3},
  pages={031043},
  year={2018},
  doi = {10.1103/PhysRevX.8.031043},
  publisher={APS}
}

@article{cui2019twin,
  title={Twin-field quantum key distribution without phase postselection},
  author={Cui, Chaohan and Yin, Zhen-Qiang and Wang, Rong and Chen, Wei and Wang, Shuang and Guo, Guang-Can and Han, Zheng-Fu},
  journal={Physical Review Applied},
  volume={11},
  number={3},
  pages={034053},
  year={2019},
  doi = {10.1103/PhysRevApplied.11.034053},
  publisher={APS}
}

@article{lu2019practical,
  title={Practical issues of twin-field quantum key distribution},
  author={Lu, Feng-Yu and Yin, Zhen-Qiang and Wang, Rong and Fan-Yuan, Guan-Jie and Wang, Shuang and He, De-Yong and Chen, Wei and Huang, Wei and Xu, Bing-Jie and Guo, Guang-Can, and others},
  journal={New Journal of Physics},
  volume={21},
  number={12},
  pages={123030},
  year={2019},
  doi = {10.1088/1367-2630/ab5a97},
  publisher={IOP Publishing}
}

@article{wang2018twin,
  title={Twin-field quantum key distribution with large misalignment error},
  author={Wang, Xiang-Bin and Yu, Zong-Wen and Hu, Xiao-Long},
  journal={Physical Review A},
  volume={98},
  number={6},
  pages={062323},
  year={2018},
  doi = {10.1103/PhysRevA.98.062323},
  publisher={APS}
}

@article{xu2020sending,
  title={Sending-or-not-sending twin-field quantum key distribution: Breaking the direct transmission key rate},
  author={Xu, Hai and Yu, Zong-Wen and Jiang, Cong and Hu, Xiao-Long and Wang, Xiang-Bin},
  journal={Physical Review A},
  volume={101},
  number={4},
  pages={042330},
  year={2020},
  doi = {10.1103/PhysRevA.101.042330},
  publisher={APS}
}

@article{wang2019beating,
  title={Beating the fundamental rate-distance limit in a proof-of-principle quantum key distribution system},
  author={Wang, Shuang and He, De-Yong and Yin, Zhen-Qiang and Lu, Feng-Yu and Cui, Chao-Han and Chen, Wei and Zhou, Zheng and Guo, Guang-Can and Han, Zheng-Fu},
  journal={Physical Review X},
  volume={9},
  number={2},
  pages={021046},
  year={2019},
  doi = {10.1103/PhysRevX.9.021046},
  publisher={APS}
}

@article{fang2020implementation,
  title={Implementation of quantum key distribution surpassing the linear rate-transmittance bound},
  author={Fang, Xiao-Tian and Zeng, Pei and Liu, Hui and Zou, Mi and Wu, Weijie and Tang, Yan-Lin and Sheng, Ying-Jie and Xiang, Yao and Zhang, Weijun and Li, Hao and others},
  journal={Nature Photonics},
  volume={14},
  number={7},
  pages={422--425},
  year={2020},
  doi={10.1038/s41566-020-0599-8},
  publisher={Nature Publishing Group UK London}
}

@article{chen2020sending,
  title={Sending-or-not-sending with independent lasers: Secure twin-field quantum key distribution over 509 km},
  author={Chen, Jiu-Peng and Zhang, Chi and Liu, Yang and Jiang, Cong and Zhang, Weijun and Hu, Xiao-Long and Guan, Jian-Yu and Yu, Zong-Wen and Xu, Hai and Lin, Jin and others},
  journal={Physical review letters},
  volume={124},
  number={7},
  pages={070501},
  year={2020},
  doi = {10.1103/PhysRevLett.124.070501},
  publisher={APS}
}


@article{Kraus,
  title = {Lower and Upper Bounds on the Secret-Key Rate for Quantum Key Distribution Protocols Using One-Way Classical Communication},
  author = {Kraus, B. and Gisin, N. and Renner, R.},
  journal = {Phys. Rev. Lett.},
  volume = {95},
  issue = {8},
  pages = {080501},
  numpages = {4},
  year = {2005},
  month = {Aug},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.95.080501},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.95.080501}
}


